Fashion is Taking Shape: Understanding Clothing Preference Based on Body Shape From Online Sources

To study the correlation between clothing garments and body shape, we collected a new dataset (Fashion Takes Shape), which includes images of users with clothing category annotations. We employ our multi-photo approach to estimate body shapes of each user and build a conditional model of clothing categories given body-shape. We demonstrate that in real-world data, clothing categories and body-shapes are correlated and show that our multi-photo approach leads to a better predictive model for clothing categories compared to models based on single-view shape estimates or manually annotated body types. We see our method as the first step towards the large-scale understanding of clothing preferences from body shape.

==> Results.tex <==
\vspace{-1cm}
\section{Qualitative Results on Shape Estimation}
\begin{figure}[h]
 \centering
\includegraphics[width=0.9\linewidth,keepaspectratio]{figures/qu3_v4.png}\vspace{0.25cm}\\
\includegraphics[width=0.9\linewidth,keepaspectratio]{figures/real_compressed_yellow}
\caption{Shape estimation results on real data. Note that the shape estimates obtained with SMPLify~\cite{smplify} are rather close to the average body shape whereas our multi-photo approach is able to recover shape details more accurately both for above-average (rows 1 and 2) and average (rows 3 and 4) body types.}\label{fig:res_real}
\end{figure}
In \autoref{fig:res_real} we present example results obtained with our method and compare it to the result obtained with SMPLify~\cite{smplify}. SMPLify fits the body model based on 2D positions of body joints that often do not provide enough information regarding body girth. This leads to shape estimates that are rather close to the average body shape for above-average body sizes (rows 1 and 2 in \autoref{fig:res_real}). SMLPify also occasionally fails to select the correct depth that results in body shape that is too tall and has bent knees (red box). The single-view variant of our approach improves over the result of SIMPLify for the first example in \autoref{fig:res_real}. However it still fails to estimate the fine-grained pose details such as orientation of the feet (blue box). In the second example in \autoref{fig:res_real} the body segmentation includes a handbag resulting in a shape estimate with exaggerated girth by our single-view approach (yellow box). These mistakes are corrected by our multi-photo approach that is able to improve feet orientation in the first example (blue box) and body shape in the second example (yellow box).
\section{Conclusion}
In this paper we aimed to understand the connection between body shapes and clothing preferences by collecting and analyzing a large database of fashion photographs with annotated clothing categories. Our results demonstrate that clothing preferences and body shapes are correlated and that we can build predictive models for clothing categories based on the output of automatic shape estimation. To obtain estimates of 3D shape we proposed a new approach that incorporates evidence from multiple photographs and body segmentation and is more accurate than popular recent SMPLify approach ~\cite{smplify}. We are making our data and code available for research purposes.
%In the future we plan to further explore the applications of our approach for clothing recommendation and incorporate other types of evidence such as semantic clothing segmentation~\cite{6751549} and fine-grained pose estimation~\cite{Guler2018DensePose}. 
\newpage
